Leveraging Adversarial Examples to Quantify Membership Information Leakage

The use of personal data for training machine learning systems comes with a privacy threat and measuring the level of privacy of a model is one of the major challenges in machine learning today. Identifying training data based on a trained model is a standard way of measuring the privacy risks induced by the model. We develop a novel approach to address the problem of membership inference in pattern recognition models, relying on information provided by adversarial examples. The strategy we propose consists of measuring the magnitude of a perturbation necessary to build an adversarial example. Indeed, we argue that this quantity reflects the likelihood of belonging to the training data. Extensive numerical experiments on multivariate data and an array of state-of-the-art target models show that our method performs comparable or even outperforms state-of-the-art strategies, but without requiring any additional training samples.

==> defense.tex <==
As described in Section \ref{}, the MIA strategy designed leverages the information provided by the amount of noise required to the adversarial attack.

Algorithm~\ref{alg:algo_defense} 
\begin{algorithm}[!h]
\caption{Land mining the }
\algsetup{linenodelimiter=.}
%\begin{algorithmic}[1]
%\end{algorithmic}


\label{alg:algo_defense}
\end{algorithm}

==> theoreticalAnalysis.tex <==
%  Assume that some prior knowledge concerning the test set is provided and the probability $\PP{S \in \mathcal{D}_\text{train}}$ of $S$ belonging to the train set is known. Let $V \in \mathcal{X}$ be the injected noise to the sample $S$ such that $\widehat{g}(S + V) \not = \widehat{g}(S)$ almost surely.
%$V$ appears to be a random quantity as its designed as two random quantities a random radius $R$ corresponding to the minimum distance required to change label for the classifier $\widehat g$ following the random direction $\tilde{U}(X) \in \mathcal{X}$ which is obtained by SGD \cite{}.
%Similarly to \cite{}, we shall assume that the true direction at a given sample $x$ is provided by
%\begin{align*}
%  \EE{\tilde U(x)} = U(x)
%\end{align*}
%)\hamid{For now, we work with the true direction for the sake of simplicity.}
%Let $V_1, \ldots, V_n$ be the random injected noise to samples $X_1, \ldots, X_n$ such that $\widehat{g}(X_1 + V_1) \not = \widehat{g}(X_1)$ almost surely. In the remaining of this paper, we shall assume that the injected noise $V$ is a random variable depending on $X$ and $g$ as the


The following proposition/theorem provides overwhelming guarantees concerning

%\begin{theorem}
%\begin{align*}
%| \mathfrak{R}(\phi, \widehat{g}) - \widehat{\mathfrak{R}}(\phi, \widehat{g}) | \leq \cdots
  %\sum_{i=1}^m \un\{X_i \in \mathcal{D}_{\text{train}}, \|V_i\| \geq \tau \} - \PP{\|V\| \geq \tau , S \in \mathcal{D}_{\text{train}}  }
%\end{align*}
%\end{theorem}
%\begin{proof}
%  \begin{align*}
%  &| \mathfrak{R}(\phi, \widehat{g}) - \widehat{\mathfrak{R}}(\phi, \widehat{g}) | \leq \\
%  &\left|\frac{1}{m}\sum_{i=1}^m \un\{\|V_i \|  \geq \tau, X_i \not \in \mathcal{D}_\text{train} \} - \PP{\phi_g(S) = 1, T=0} \right| + \\
%  &\left|\frac{1}{m}\sum_{i=1}^m \un\{\|V_i \|  < \tau, X_i \in \mathcal{D}_\text{train} \} - \PP{\phi_g(S) = 0, T=1} \right|
    %\sum_{i=1}^m \un\{X_i \in \mathcal{D}_{\text{train}}, \|V_i\| \geq \tau \} - \PP{\|V\| \geq \tau , S \in \mathcal{D}_{\text{train}}  }
%  \end{align*}
%\end{proof}
%\hamid{I can control both terms up to making assumptions that we shall discuss.}

